Approximate Query Service on Autonomous IoT Cameras

Elf is a runtime for an energy-constrained camera to continuously summarize video scenes as approximate object counts. Elf's novelty centers on planning the camera's count actions under energy constraint. (1) Elf explores the rich action space spanned by the number of sample image frames and the choice of per-frame object counters; it unifies errors from both sources into one single bounded error. (2) To decide count actions at run time, Elf employs a learning-based planner, jointly optimizing for past and future videos without delaying result materialization. Tested with more than 1,000 hours of videos and under realistic energy constraints, Elf continuously generates object counts within only 11% of the true counts on average. Alongside the counts, Elf presents narrow errors shown to be bounded and up to 3.4x smaller than competitive baselines. At a higher level, Elf makes a case for advancing the geographic frontier of video analytics.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


==> design-RL.old.tex <==
% !TeX root = main.tex

\subsection{The RL-based Online Planner}\label{sec:design:rl}

\input{fig-rl}

\paragraph{Overview}
In this section, we introduce our deep reinforcement learning based approach for sampling. 
For each camera, we first collect several days (e.g., 3) of video data.
Then we run the oracle planner repeatedly on each video to generate a simulated dataset, on which, we train RL agents to imitate oracle planner's behavior.
After the training is completed, we can deploy the RL agents to make on-the-go sampling decision.

\paragraph{Design Rationale}
%The oracle allocator can only solve the sampling problem with complete information of each window at the end of the planning horizon, which results in undesirable delay.



In each \planwindow{}, \sys{} has to make a series of decisions to minimize the mean CI width.
Furthermore, to deliver timely results, \sys{} has to make these decisions before each \aggwindow.
This is a typical sequential decision making problem.
And we do not have a perfect model for the environment.
Rather than handcrafting a heuristics-based algorithm and tuning it for each camera, we leverage deep reinfocement learning (RL) to learn a sampling strategy for each camera.


% This problem is essentially difficult. Because \sys{} has to make these decisions under incomplete information. 
% Under the overall energy budget, processing more frames for the current window means less energy in the future. But who knows what will happen in the future? 

% To solve this non-trivial problem,
%instead of making independent decisions for each window,
% we leverage deep reinfocement learning (RL) to learn a sampling strategy. \Note{justification}
% However, it's infeasible to directly apply RL to solve the energy allocation problem for three reasons.

% \Note{means what?}
% Second, the rewards are usually delayed until the end of each planning horizon. 
% \Note{means what?}
% Only after each \planwindow, we can evaluate how well the agent performs to decide the reward or punishment correspondingly. %The sparsity makes the training difficult.
% Third, the energy budget for \sys{} is a hard constraint involving multiple steps. \Note{total outcome shall respect a global budget... accumulative resource consumption...}
% And there is no good way to enforce such hard constraint in existing RL algorithms.


However, to  learn a on-the-go sampling decision engine, we have the following challenges.
\begin{myitemize}
	\item A \planwindow{} often contains tens of \aggwindow s (48 in default), and this joint decision space is extremely large and difficult to explore by an RL agent. 
	\item Only after each \planwindow, we can evaluate how well the agent performs to decide the reward or punishment correspondingly, which results in long delay of reward signals.
	\item The accumulative energy consumption of a \planwindow{} should respect the predefined energy budget, which is a hard constraint involving multiple steps. And there is no good way to enforce such a hard constraint in existing RL algorithms.
\end{myitemize}

\Note{Highlight key ideas or principles}

So, instead of directly applying RL, we train two separate RL agents to imitate the behavior of oracle allocator, which overcomes the above challenges.
\begin{myitemize}
	\item Rather than considering the global energy planning directly, the agents only need to imitate the oracle allocator on the current window. As the joint decision space is decoupled, the problem becomes much simpler for the agents.
	\item At every step, we can punish the RL agents by how much they deviate from the oracle planner's decisions, which results in timely and frequent reward signals.
	\item By learning the strategy of the oracle allocator, who strictly follows the energy budget, the RL agents can also learn the contraint (energy budget) implicitly. 
	
% \item mimic the behaviors of oracle...
% We note that recent RL-based systems do not do this... (they learn from the outcome/quality of the action, instead of the deviation from the oracle...)
% \item two agents... 
% this addresses C1...
\end{myitemize}

% This approach has several benefits.
% First, rather than considering the global energy planning directly, the agents only need to imitate the oracle allocator on the current window. \Note{highlight this}
% As the joint decision space is decoupled, the problem becomes much simpler for the agents.
% Second, at every step, if the decision by the RL agent deviates from the decisions by the oracle allocator, we can punish it correspondingly. 
% In such a way RL agent receives more frequent rewards. \Note{isn't this generic RL?} 
% Third, by learning the strategy of the oracle allocator, who strictly follows the energy budget, the RL agent can also learn the contraint (energy budget) implicitly. 
% \st{Our experiment results also prove this.}

%\paragraph{Problem formulation}

%By reinforcement learning (RL), \sys{} attempts to learn an online decision maker from observations about offline energy allocation.
%RL considers a general setting in which an agent interacts with an environment.
%At each time step $t$, the agent observes some state $s_t$, and chooses an action $a_t$.
%After applying the action, the state of the environment transitions to $s_{t+1}$ and the agent receives a reward $r_t$ .
%The goal of learning is to maximize the expected cumulative discounted reward: %$E(\sum_{t=0}^{\infty}\gamma^tr_t)$, where
%$\gamma \in (0, 1]$ is a factor discounting future rewards.

%\textbf{RL design} FigureXXX summarizes how RL is applied in \sys.
%The decision maker (agent) observes a set of metrics, including the energy budget, the online processing results from previous $N$ {\aggwindow}s (states) and feeds them to the neural network.
%Then the neural network outputs the decision (action), i.e., the number of frames to capture and the NN detector to use.
% \note{what's the reward}?

% \note{We shall be more conservative? Capture more?}

\Note{useful but we probably dont have space}

\paragraph{RL primer}
Generally, an RL agent interacts with its environment in discrete time steps to maximize its cumulative reward. 
The environment, that it interacts with, can be formally described as a Markov Decision Process (MDP). A MDP is defined by a tuple $\{S, A, P_{s,a}, r\} $, where 

\begin{myitemize}
	\item 
	$S$ is the state space (discrete or continuous).
	\item 
	$A$ is the action space (discrete or continuous).
	\item 
	$P_{s,a}=p(s_{t+1}|s_t,a_t)$ are the state transition probabilities.
	\item 
	$r: S \times A \mapsto \mathbb{R} $ is the reward function.
\end{myitemize}

If the environment is fully observable, at each time step $t$, based on the current state $s_t \in S$ of the environment, the agent can take an action $a_t \in A$. 
Then, the environment transitions from $s_t$ to $s_{t+1}$ and sends a corresponding reward $r_t$ to the agent. 
However, if the environment is only partially observable, at each time step, instead of the state $s_t$, the agent can only receive an observation $o_t$ from the environment, and take an action based on the observation.

\Note{clarify what happens online, what happens ahead of time}
\Note{training: paragraph 1\&2, online: paragraph 3}

\paragraph{RL Design}
Fig \ref{fig:rl} shows how the RL agents are trained to imitate the oracle energy allocator.
In our scenario, a time step is defined as an aggregation window. 
Before each aggregation window, two heterogeneous decisions have to made, how many frames to capture (continuous), and which operator to use (discrete).
So we train two RL agents, a regression agent and a classification agent, responsible for each decision respectively.

Before window $W_t$, each agent receives an observation vector $o_t$, containing the mean object counts in the past windows.
% \Note{why 4}, $\{W_{t-4},W_{t-3},W_{t-2},W_{t-1}\}$. 
Based on the observation, the classification agent predicts the NN counter to use, $NN_{t,agent}$, while the regression agent predict the number of frames to process, $f_{t,agent}$.
Then, the decisions by the agents are compared with those by the oracle planner, and the reward signal for each agent is computed correspondingly.

After training is completed, only the two agents are deployed to the camera, whih are essentially two very small neural networks. 
And before each \aggwindow, \sys{} runs each neural network agent once to get the sampling decision.
Because the agents can only imitate the oracle approximately, to avoid running out of energy before the horizon end, \sys{} keeps monitoring remaining energy.
Anytime when the remaining energy is only enough for processing 30/XX frames per future window with the cheapest NN operator, \sys{} stops relying on RL agents and follows the minimum sampling plan until the end of horizon.
 

Specifically, the reward function for the regression agent is defined as
$$ r_{t,regression} = - | f_{t,agent} - f_{t,oracle} | $$
where $f_{t,oracle}$ is the number of frames to capture decided by the oracle allocator, while the reward function for the classification agent is defined by the following formula,
\begin{equation}\nonumber
	r_{t,classification} =
	\begin{cases}
	0& NN_{t,agent} \neq NN_{t,oracle}\\
	1& NN_{t,agent} = NN_{t,oracle}
	\end{cases}
	\end{equation}
where $NN_{t,oracle}$ is the NN counter chosen by oracle allocator.



\paragraph{RL Training}
We adopt the Actor-Critic framework\note{cite} to train the agents. 
Specifically, we use A2C~\cite{a2c} as our training algorithm, a synchronous, deterministic variants of the A3C algorithm~\cite{a3c}. 
There are two neural network approximators used in the Actor-Critic framework: an actor neural network representing the policy, and a critic neural network constantly evaluating the actor's performance to facilitate training. 
The actor-critic algorithm used here is a policy gradient method. 
Every iteration, the policy is updated by the following formula.
$$\theta \leftarrow \theta + \alpha \sum_t \nabla_\theta log \pi_\theta (o_t, a_t) A^{\pi_\theta}(o_t, a_t)$$
where $\alpha$ is the learning rate, $\theta$ represents the parameters of the actor neural network, $\pi_\theta(o_t,a_t)$ represents the current policy of the actor, and $A^{\pi_\theta}(o_t,a_t) = Q^{\pi_\theta}(o_t,a_t) - V^{\pi_\theta}(o_t)$ is the advantage function, which encodes how much better a specific action is. The action-value function $Q^{\pi_\theta(o_t,a_t)}(o_t,a_t)$, also called the Q-value, is estimated by the critic neural network, and the state-value function, $V^{\pi_\theta}(o_t) = \sum_{a \in A} \pi_\theta(o_t,a_t) Q^{\pi_\theta}(o_t,a_t)$, represents the expected cumulative reward of $\pi_{\theta}$ starting from $o_t$.

\Note{could go to Sec impl}

The neural network architecture we adopt here is a multi-layer perceptron (MLP). For both the regression agent and the classification agent, we use a MLP with 2 hidden layers. The input layer has 4 input units, while two hidden layers each have 64 hidden units. 

Usually, it takes more than 100000 steps for the training to converge, which means about 2000 days of training data. Training agents in such a way is infeasible. To overcome this difficulty, for one camera, we first collect \note{4-7} days. Then, we simulate a training enviornment for the agents by playing the collected video repeatedly.
\note{We also change the environments (energy budget) during repeat training.}

\paragraph{What the RL has learnt?}
The RL agents learn to predict next window's video characteristics from the observation on previous windows.
They learn the dynamics of the object count in the video from their past observation, so that they can make decisions about how many frames to sample and which NN counter to use. 
By imitating the oracle planner, the agents also learn the global energy budget and the energy/CI front of each window implicitly.
Also, the error of each NN counter is implicitly learnt when constructing the CIs as discussed in $\S$\ref{sec:design-CI}.
Noting that the error of the same NN counter can be different across different videos, our RL algorithm is customized for each video stream.

\paragraph{On-camera overhead of RL: negligable}
The agent network has approximately 4,545 parameters and performs 4,416 multiply-adds operations, while the most lightweight NN counter in our operator library, MobileNetV2 + SSDLite, has about 4.3 million parameters and performs 0.8 billion multiply-adds operations. 
Furthermore, {\sys } processes at least 30 frames in every window, while it only needs to run each agent network once before every aggregation window.
Therefore, the energy consumption of the RL agents is negligable: contributing to $<0.0001\%$ of the total energy budget.



% To generate the online decision maker, \sys{} runs a training phase at the first $K$ days after camera installation.
% Ideally, training a RL model requires a large number of steps, e.g., thousands or even millions.
% It will takes hundreds of days to collect enough training data given that camera only goes through 48 {\aggwindow}s each day ($w=30mins$).

%To accelerate this process, \sys{} repetitively trains the RL model based on the data from the same $K$ days, but assigned with different energy budgets or target CIs within a reasonable range, e.g., 10Wh $\sim$ 30Wh per day.


%\paragraph{RL overhead on camera}

==> design-RL.orig.tex <==
% !TeX root = main.tex

\subsection{The RL-based Online Planner}\label{sec:design:rl}

\input{fig-rl}

\note{In offline training, we can run all the NNs exhaustively to get the energy/CI fronts.}

\paragraph{Overview}
For each camera, \sys{} first runs the oracle planner on several days (e.g., 3) of video data.
\sys{} then trains an RL agent based on the sampling decision \{<N,C>\} made by the oracle planner.
The environment of the RL agent includes the energy budget and the sampling outcome of previous {\aggwindow}s.
Finally, \sys{} deploys the RL agent to make on-the-go sampling decision.

\paragraph{Why RL?}
RL is known to be good at taking step-by-step actions (decisions) based on the observable environments,
Generally, an RL agent interacts with its environment in discrete time steps to maximize its cumulative reward. 
The environment, that it interacts with, can be formally described as a Markov Decision Process (MDP). A MDP is defined by a tuple $\{S, A, P_{s,a}, r\} $, where 

\begin{myitemize}
	\item 
	$S$ is the state space (discrete or continuous).
	\item 
	$A$ is the action space (discrete or continuous).
	\item 
	$P_{s,a}=p(s_{t+1}|s_t,a_t)$ are the state transition probabilities.
	\item 
	$r: S \times A \mapsto \mathbb{R} $ is the reward function.
\end{myitemize}

If the environment is fully observable, at each time step $t$, based on the current state $s_t \in S$ of the environment, the agent can take an action $a_t \in A$. 
Then, the environment transitions from $s_t$ to $s_{t+1}$ and sends a corresponding reward $r_t$ to the agent. 
However, if the environment is only partially observable, at each time step, instead of the state $s_t$, the agent can only receive an observation $o_t$ from the environment, and take an action based on the observation.

%\paragraph{Challenges}
\paragraph{Rationale}
RL is known to be good at taking step-by-step actions (decisions) based on the observable environments, instead of a long-term global planning.
\Note{A straightforward application of RL does not work...}
The oracle planner, however, helps decompose the problem of global energy planning into a single sampling decision at each {\aggwindow}s.
It also greatly increases the rewarding frequency, from one in per \planwindow{} to per \aggwindow, making the RL training easier and more feasible.

\Note{this is opportunity}
Another critical part of building a workable RL agent is to identify the environment that has strong causality with the expected actions (sampling decision).
As discussed in $\S$\ref{sec:overview:problem}, the global energy planning mainly depends on the energy/CI fronts, which are derived from the video characteristics (object count and count variation).
As we observed, the video characteristics at consecutive windows often have temporal locality.
In other words, the sampling outcome of previous {\aggwindow}s as RL environment
are both observable (on-the-go sampling) and useful (temporal pattern).

\paragraph{What the RL has learnt?}
The RL agents learn to predict next window's video characteristics from the observation on previous windows.
They learn the dynamics of the object count in the video from their past observation, so that they can make decisions about how many frames to sample and which NN counter to use. 
By imitating the oracle planner, the agents also learn the global energy budget and the energy/CI front of each window implicitly.
Also, the error of each NN counter is implicitly learnt when constructing the CIs as discussed in $\S$\ref{sec:design-CI}.
Noting that the error of the same NN counter can be different across different videos, our RL algorithm is customized for each video stream.

\begin{comment} -- by xiwen
\Note{------------------}
In each \planwindow{}, \sys{} has to make a series of decisions to minimize the mean CI width.
Furthermore, to deliver timely results, \sys{} has to make these decisions before each \aggwindow.
This is a typical sequential decision making problem.
And we do not have a perfect model for the environment.
Rather than handcrafting a heuristics-based algorithm and tuning it for each camera, we leverage deep reinfocement learning (RL) to learn a sampling strategy for each camera.

However, to  learn a on-the-go sampling decision engine, we have the following challenges.
\begin{myitemize}
	\item A \planwindow{} often contains tens of \aggwindow s (48 in default), and this joint decision space is extremely large and difficult to explore by an RL agent. 
	\item Only after each \planwindow, we can evaluate how well the agent performs to decide the reward or punishment correspondingly, which results in long delay of reward signals.
	\item The accumulative energy consumption of a \planwindow{} should respect the predefined energy budget, which is a hard constraint involving multiple steps. And there is no good way to enforce such a hard constraint in existing RL algorithms.
\end{myitemize}

So, instead of directly applying RL, we train two separate RL agents to imitate the behavior of oracle allocator, which overcomes the above challenges.
\begin{myitemize}
	\item Rather than considering the global energy planning directly, the agents only need to imitate the oracle allocator on the current window. As the joint decision space is decoupled, the problem becomes much simpler for the agents.
	\item At every step, we can punish the RL agents by how much they deviate from the oracle planner's decisions, which results in timely and frequent reward signals.
	\item By learning the strategy of the oracle allocator, who strictly follows the energy budget, the RL agents can also learn the contraint (energy budget) implicitly. 
\end{myitemize}

\Note{------------------}

% This approach has several benefits.
% First, rather than considering the global energy planning directly, the agents only need to imitate the oracle allocator on the current window. \Note{highlight this}
% As the joint decision space is decoupled, the problem becomes much simpler for the agents.
% Second, at every step, if the decision by the RL agent deviates from the decisions by the oracle allocator, we can punish it correspondingly. 
% In such a way RL agent receives more frequent rewards. \Note{isn't this generic RL?} 
% Third, by learning the strategy of the oracle allocator, who strictly follows the energy budget, the RL agent can also learn the contraint (energy budget) implicitly. 
% \st{Our experiment results also prove this.}

%\paragraph{Problem formulation}

%By reinforcement learning (RL), \sys{} attempts to learn an online decision maker from observations about offline energy allocation.
%RL considers a general setting in which an agent interacts with an environment.
%At each time step $t$, the agent observes some state $s_t$, and chooses an action $a_t$.
%After applying the action, the state of the environment transitions to $s_{t+1}$ and the agent receives a reward $r_t$ .
%The goal of learning is to maximize the expected cumulative discounted reward: %$E(\sum_{t=0}^{\infty}\gamma^tr_t)$, where
%$\gamma \in (0, 1]$ is a factor discounting future rewards.

%\textbf{RL design} FigureXXX summarizes how RL is applied in \sys.
%The decision maker (agent) observes a set of metrics, including the energy budget, the online processing results from previous $N$ {\aggwindow}s (states) and feeds them to the neural network.
%Then the neural network outputs the decision (action), i.e., the number of frames to capture and the NN detector to use.
% \note{what's the reward}?

% \note{We shall be more conservative? Capture more?}

\end{comment}



\paragraph{Formulation}
\Note{formulate:}
what is timestep? agents? observation? what is reward? how to feed different energy budgets?

\paragraph{RL Design - offline training}
Figure~\ref{fig:rl} shows how the RL agents are trained to imitate the oracle energy allocator.
In our scenario, a time step is defined as an aggregation window. 
\Note{extract as a design point}
Before each aggregation window, two heterogeneous decisions have to made, how many frames to capture\&process (continuous), and which operator to use (discrete).
So we train two RL agents, a regression agent and a classification agent, responsible for each decision respectively.


Before window $W_t$, each agent receives an observation vector $o_t$, containing the mean object counts in the past windows.
% \Note{why 4}, $\{W_{t-4},W_{t-3},W_{t-2},W_{t-1}\}$. 
Based on the observation, the classification agent predicts the NN counter to use, $NN_{t,agent}$, while the regression agent predict the number of frames to process, $f_{t,agent}$.
Then, the decisions by the agents are compared with those by the oracle planner, and the reward signal for each agent is computed correspondingly.

\Note{the following may be omitted}
We adopt the Actor-Critic framework\note{cite} to train the agents. 
Specifically, we use A2C~\cite{a2c} as our training algorithm, a synchronous, deterministic variants of the A3C algorithm~\cite{a3c}. 
There are two neural network approximators used in the Actor-Critic framework: an actor neural network representing the policy, and a critic neural network constantly evaluating the actor's performance to facilitate training. 
The actor-critic algorithm used here is a policy gradient method. 
Every iteration, the policy is updated by the following formula.
$$\theta \leftarrow \theta + \alpha \sum_t \nabla_\theta log \pi_\theta (o_t, a_t) A^{\pi_\theta}(o_t, a_t)$$
where $\alpha$ is the learning rate, $\theta$ represents the parameters of the actor neural network, $\pi_\theta(o_t,a_t)$ represents the current policy of the actor, and $A^{\pi_\theta}(o_t,a_t) = Q^{\pi_\theta}(o_t,a_t) - V^{\pi_\theta}(o_t)$ is the advantage function, which encodes how much better a specific action is. The action-value function $Q^{\pi_\theta(o_t,a_t)}(o_t,a_t)$, also called the Q-value, is estimated by the critic neural network, and the state-value function, $V^{\pi_\theta}(o_t) = \sum_{a \in A} \pi_\theta(o_t,a_t) Q^{\pi_\theta}(o_t,a_t)$, represents the expected cumulative reward of $\pi_{\theta}$ starting from $o_t$.

\Note{could go to Sec impl}

The neural network architecture we adopt here is a multi-layer perceptron (MLP). For both the regression agent and the classification agent, we use a MLP with 2 hidden layers. The input layer has 4 input units, while two hidden layers each have 64 hidden units. 

Usually, it takes more than 100000 steps for the training to converge, which means about 2000 days of training data. Training agents in such a way is infeasible. To overcome this difficulty, for one camera, we first collect \note{4-7} days. Then, we simulate a training enviornment for the agents by playing the collected video repeatedly.
\note{We also change the environments (energy budget) during repeat training.}
 

% Specifically, the reward function for the regression agent is defined as
% $$ r_{t,regression} = - | f_{t,agent} - f_{t,oracle} | $$
% where $f_{t,oracle}$ is the number of frames to capture decided by the oracle allocator, while the reward function for the classification agent is defined by the following formula,
% \begin{equation}\nonumber
% r_{t,classification} =
% \begin{cases}
% 0& NN_{t,agent} \neq NN_{t,oracle}\\
% 1& NN_{t,agent} = NN_{t,oracle}
% \end{cases}
% \end{equation}
% where $NN_{t,oracle}$ is the NN counter chosen by oracle allocator.

%\paragraph{RL Design - online deployment}
\paragraph{Online prediction (?)}
After training is completed, only the two agents are deployed to the camera.
Before each \aggwindow, \sys{} runs each agent once to get the sampling decision. 
The processing results are used to
i) materialize the aggregated counts and CI as will be discussed in $\S$\ref{sec:design-CI}, and
ii) guide the sampling decision in next \aggwindow.

\Note{The ``backstop'' ... what if RL mispredicts... Goal is to avoid no counts for certain windows. CI becomes infinite}
From the scope of \planwindow, \sys{} may under/over-utilize the energy budget.
To stay energy neutral, \sys{} keeps monitoring the energy balance as the remainder from the budget. 
Anytime when the remaining energy is only enough for processing 30 frames per future window with the cheapest NN counter, \sys{} stops relying on RL agents and follows the minimum sampling plan during the rest of the \planwindow.
At the end of the \planwindow, if the energy budget is under-utilized, the unexploited energy will be added to the next \planwindow{} as done by prior work~\cite{farmbeats};



\paragraph{On-camera overhead of RL: negligable}
The agent network has approximately 4,545 parameters and performs 4,416 multiply-adds operations, while the most lightweight NN counter in our operator library, MobileNetV2 + SSDLite, has about 4.3 million parameters and performs 0.8 billion multiply-adds operations. 
Furthermore, {\sys } processes at least 30 frames in every window, while it only needs to run each agent network once before every aggregation window.
Therefore, the energy consumption of the RL agents is negligable: contributing to $<0.0001\%$ of the total energy budget.



% To generate the online decision maker, \sys{} runs a training phase at the first $K$ days after camera installation.
% Ideally, training a RL model requires a large number of steps, e.g., thousands or even millions.
% It will takes hundreds of days to collect enough training data given that camera only goes through 48 {\aggwindow}s each day ($w=30mins$).

%To accelerate this process, \sys{} repetitively trains the RL model based on the data from the same $K$ days, but assigned with different energy budgets or target CIs within a reasonable range, e.g., 10Wh $\sim$ 30Wh per day.


%\paragraph{RL overhead on camera}

==> eval-adapt.tex <==
\subsection{How \sys{} Adapts to Varying Energy}\label{sec:eval-adapt}

\input{fig-eval-adapt}

We then study how \sys{} performs under changing environments.
We run \sys{} on two videos, Jackson and Cross, with the energy budget gradually drops from 30Wh/day to 10Wh/day.
We report the mean CI width on every two days with and without renewing the knowledge ($\S$\ref{sec:plan:backward}).

As shown in Figure~\ref{fig:eval-adapt}, {\sys}'s performance drops as the energy budget becomes tighter on both videos due to the reduced number of processed frames.
However, with {\sys}'s adaptiveness through knowledge renewing, the mean CI width only increases by 7.4\% and 5.4\% on Jackson and Cross, respectively.
Turning off the adaptiveness, the mean CI width increases become 8.3\% and 9.9\%.
As we observed, the main difference is that, without adapting to the reducing energy budget, \sys{} captures excessive frames during but has no enough energy to process them.
% As a result, the energy to capture those unprocessed frames are wasted.

==> fig-capture.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
	\includegraphics[width=0.35\textwidth]{figs/eval/capture}
	%\vspace*{-.6cm}
	\caption{
\sys{} still consumes less energy than alternatives as the frame capture cost increases. 	
Note: \OptOp{} is an idealistic, impractical design as explained in \S\ref{sec:eval-method}.
	Video: Hampton; CI target: 20\%.}
	\label{fig:eval-capture}
\end{figure}



==> fig-components.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{figs/components}
	%\vspace*{-.6cm}
	\caption{Components of \sys{}.}
	\label{fig:components}
\end{figure}



==> fig-eval-adapt.tex <==
\begin{figure}
	\centering					
	\begin{minipage}[b]{0.44\textwidth}
		\includegraphics[width=1\textwidth]{figs/eval/perf-adapt-jackson.pdf}
		\subcaption{Jackson}
	\end{minipage}


	\centering					
	\begin{minipage}[b]{0.44\textwidth}
		\includegraphics[width=1\textwidth]{figs/eval/perf-adapt-cross.pdf}
		\subcaption{Cross}
	\end{minipage}
	
	\caption{Without renewing its knowledge to changing environment, \sys{}'s performance drops across time.}
	\label{fig:eval-adapt}
\end{figure}

==> fig-eval-design.tex <==
% !TeX root = main.tex
\begin{figure}
	\centering					
	\begin{minipage}[b]{0.24\textwidth}
		\includegraphics[width=1\textwidth]{figs/eval-design-sample.png}
		\subcaption{video 1}
	\end{minipage}	
	~			
	\centering				
	\begin{minipage}[b]{0.24\textwidth}
		\includegraphics[width=1\textwidth]{figs/eval-design-sample.png}
		\subcaption{video 2}
	\end{minipage}


	\centering					
	\begin{minipage}[b]{0.24\textwidth}
		\includegraphics[width=1\textwidth]{figs/eval-design-sample.png}
		\subcaption{Video 3}
	\end{minipage}	
	~			
	\centering				
	\begin{minipage}[b]{0.24\textwidth}
		\includegraphics[width=1\textwidth]{figs/eval-design-sample.png}
		\subcaption{Video 4}
	\end{minipage}
	
	\caption{Validation of {\sys}'s key designs.}
	\label{fig:eval-design}
\end{figure}

==> fig-mapping.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/mapping}
	%\vspace*{-.6cm}
	\caption{Forward (online) phase of {\sys}'s planner.}
	\label{fig:mapping}
\end{figure}

==> fig-op-std.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{figs/op-std}
	%\vspace*{-.6cm}
	\caption{Accuracy-energy trades-off of different operators.}
	\label{fig:op-std}
\end{figure}



==> figs/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> hw.tex <==
\subsection{Heterogeneous capture and processing}\label{sec:opt:hw}

The energy consumption of \sys{} mainly comes from two parts: image capture and image processing.

\textbf{Image capture energy is non-trivial}.
Traditional cameras (both commerical products and research prototypes) only use the main processing unit (e.g., CPU) to do both image capture and processing.
However, we find such design is not energy efficient for \sys{} paradigm.
According to our measurements on Raspberry Pi 3 and ssd\_mobilenet\_v2 object detector, the energy consumption to capture one frame is almost XX\% of the energy to process one.

The reasons of such high energy consumption of image capture are mainly twofolded.
(1) In \sys{}, image capture is sparse, so most of the time the whole system is kept in deep sleep to save energy. Waking up and taking a picture is slow since the camera needs to initialize the whole OS as well as the associated drivers (typically X-Y seconds on RPI 3).
Only a small fraction of energy is really paid for image sensor.
(2) \sys{} is designed to batch image processing together (during prob processing and offline scheduling in Section~\ref{sec:design-plan}). Though image processing requires substantial computing power, but the wakeup energy is amortized over tens or even hundreds of frames.

\textbf{CPU-LPU cooperation}.
To reduce the energy consumption, \sys{} deploys a CPU-LPU heterogeneous architecture.
More specifically, \sys{} uses a low power unit (e.g., micro-controller) to capture frames from time to time. During image capture, the LPU receives a self-issued interrupt, wakes up from deep sleep, asks the image sensor to capture one frame, and finally goes back to sleep. No commodity OS like Linux needs to be loaded or initialized. In our prototype of OpenMV M7, this image capture process only takes XX\% seconds to complete, consuming XX\% less energy than rpi 3.
CPU will only be waken up to process frames using operators.

==> intro-analytics-first.tex <==
% !TeX root = main.tex

\section{Introduction}\label{sec:intro}

\note{Bring up ``approximate query'' somewhere.}

% by estimating the human population in retailing store, store managers can better plan...; 
% by estimating human crowd density in public area during an event, the police department can avoid disaster.... 
%therefore enabling a variety of video analytics~\cite{yogameena2017computer,karpagavalli2013estimating, beymer1997real,lipton2015video,zhu2017online, norouzzadeh2018automatically,mongeon2017busyness}

%\paragraph{Target analytics: video summaries as object counts}
\paragraph{Video summary analytics}
Commodity IoT cameras produce large videos at low monetary costs~\cite{wyze-camv2,yi-cam}. 
To extract insights from a video scene, 
it is common to summarize the scene as \textit{object counts}:
%the analytics emits aggregated counts of object instances detected in consecutive video timespans, or windows, as shown in Figure~\ref{fig:workflow}.
as shown in Figure~\ref{fig:workflow}, 
a summary consists of a stream of object counts, one count for each video timespan called an \aggwindow{}. 
Object counts enable rich applications. 
For instance, %\Note{both are counting ppl. can we diversify?}
counting customers in retailing stores reveals customer interest and therefore guides optimization of merchandise arrangement~\cite{lipton2015video};
counting audience in sports events helps avoid crowd-related disasters~\cite{video-public-safety,karpagavalli2013estimating}.
Other applications include traffic monitoring~\cite{beymer1997real,naphade2017nvidia,liu2016highway,hsieh2017drone},
public safety~\cite{yogameena2017computer,karpagavalli2013estimating},
and wildlife study~\cite{norouzzadeh2018automatically,parham2017animal,
van2014nature,hodgson2016precision}.
%and smart retailing~\cite{lipton2015video,mongeon2017busyness,zhu2017online,store-plan}.

\paragraph{A case for autonomous cameras}
While today's IoT cameras and their analytics mostly target urban and residential areas, 
there exist rich opportunities in diverse environments where cameras stay ``off grid'' and are  connected with highly constrained networks. 
These environments include construction sites, interstate highways, underdeveloped regions, and farms. 
Examples abound: 
along interstate highways, cameras estimate traffic from vehicle counts, which is cheaper than deploying inductive loop detector~\cite{inductive-loop,liu2016highway};
on a large cattle farm, scattered cameras count cattle and therefore monitor their distribution, which is more cost-effective than making cattle wear GPS devices~\cite{IoT-cattle-tracking,digitalanimal-cattle-tracking,postscapes-cattle-tracking}.


%\Note{counter argument: why don't upload the frames to the cloud/edge since you will need network anyway?}

%\Note{connectivity is expensive; or has to be provided on demand to the cameras}

To execute video analytics in such environments, 
cameras must be \textit{autonomous}.
First, they must be energy independent.
Lacking wired power supply, they typically operate on harvested energy, e.g., solar or wind~\cite{solar-camera,solar-AI,ur-solarwind}.
Second, they must be compute independent. 
Typically on low-power wide-area network where bandwidth is low (e.g. tens of Kbps~\cite{lora}) or even intermittent, the cameras must execute video analytics on device and emit only concise summaries to the cloud. Section~\ref{sec:bkgnd} will offer more evidence. 

\input{fig-workflow}
 
%For example, by counting the number of vehicles on intersections or highways, we can monitor the traffic for better city planning~\cite{beymer1997real,naphade2017nvidia,
%liu2016highway,hsieh2017drone}.
%By counting the number of persons in shopping malls, we can achive better
%public safety~\cite{yogameena2017computer,karpagavalli2013estimating} or store plan~\cite{lipton2015video,mongeon2017busyness,
%zhu2017online,store-plan}.
%Counting the number of different kinds of wild animals can help ecologists study their behavior~\cite{norouzzadeh2018automatically,parham2017animal,
%van2014nature,hodgson2016precision}.
%We will discuss query model in detail in $\S$\ref{sec:overview:query}. 


\paragraph{\sys{} and its operation}
%To answer this question, we design \sys{}, a runtime system for \sysmodel{} to 
This paper answers the following question:
%can the frugal camera resources, especially limited energy, to execute useful analytics? 
how to manage frugal camera resources, especially limited energy, to produce useful analytics results? 
Our response is \sys{}, a runtime for an autonomous camera to continuously produce video summaries in the form of object counts. 
The counts are approximate, annotated with confidence intervals (CIs) as shown in Figure~\ref{fig:workflow}.
CI is a common notion in approximate query processing (AQP)~\cite{blinkdb,summarystore,garofalakis2001approximate,olamr,yan2014error,chakrabarti2001approximate}.
\revise{
Given the nature of approximation in video analytics, especially in the resource-constrained domain, accompanied CIs can make the ``inaccurate'' counting results more meaningful and insightful.
It also enables higher-level video queries built atop the approximation such as ``there is 90\% chance that the number of cars crossing this intersection has increased by 2 times since this week''.
A narrower CI suggests higher confidence in the count, hence more useful to users.
}

%the top goal is to best use limited energy for answering queries with highly confident results, i.e., bounded and low errors. 
%the top goal is:
% to best use limited energy for producing counts with high overall confidence, 
% e.g, with a minimum average error over a series of aggregated counts. 
% , i.e., with \textit{bounded} and \textit{low} errors. 
% to best use limited energy for producing highly confident counts, i.e., with \textit{bounded} and \textit{low} errors. \Note{clearly define goal}
%\sys{} builds on existing energy-harvesting OSes:
We build \sys{} atop periodic energy budgets, an abstraction commonly provided by existing energy-harvesting OSes~\cite{goiri2012greenhadoop,farmbeats}.
As illustrated in Figure~\ref{fig:workflow}, at fixed time intervals of a \textit{\planwindow{}} (e.g., one day), the OS replenishes energy budget to be used by \sys{} in the upcoming \planwindow{}. 
%Operating under the energy budget, \sys{} executes the analytics:
%\sys{} operates under an energy budget that is replenished periodically at time intervals called \planwindow{}s. 
%The periodic energy budget is common in energy-harvesting systems~\cite{goiri2012greenhadoop,farmbeats};
%it is often implemented by OSes for allocating energy that exhibits temporal patterns (e.g. daily solar energy) to applications. 
%giving them the essential headroom for planning energy use over long timespans. 
%To count objects, \sys{} follows periodic sampling as in prior AQP systems \Note{cite}. 
%\sys{} processes sparse samples of image frames, as shown in Figure~\ref{fig:workflow}. 
With the energy budget, 
\sys{} periodically wakes up the camera to capture video frames (\circled{1});
%At predefined (\Note{who defines?}) intervals 
it runs object counters on each of the captured frames (\circled{2});
by aggregating the per-frame object counts, 
\sys{} materializes a per-window aggregated object count for each window (\circled{3});
\sys{} emits the sequence of aggregated counts by uploading them to the cloud either in real time or upon user requests. 

\begin{comment}
\Note{merge the following}
During each \aggwindow, \sys{} periodically wakes up, captures, and stores video frames on local storage.
At the end of \aggwindow, \sys{} runs NN counters on the captured frames in \textit{batch} mode and generate aggregated counts.
All frames will be deleted once processed.
\Note{combine the following}
After materialization, \sys{} deletes all images for the $N$ windows. 
it also assures data privacy, as \sys{} never stores images older than a planning horizon.
\end{comment}

\paragraph{The central problem: count planning}
%The key challenge is to produce \Note{overall high confidence?} counts with highest confidence (i.e. lowest and bounded errors) under the energy budget.  
%To do so, \sys{} decide on sample actions: 
The theme of \sys{} is to produce aggregated object counts with high confidence under energy constraint. 
As shown in Figure~\ref{fig:workflow}(a): \sys{}'s operational objective for a \planwindow{} \myH{} is to maximize the overall confidence in all the emitted aggregated counts belonging to \myH{} while respecting the energy budget for \myH{}.
%Toward this objective, \sys{} controls count actions for individual windows in \myH{}. % each window belonging to $H$. 

%Specifically, \sys{}'s operation objective is for each \planwindow{} maximizing the overall confidence of aggregated counts while respecting the energy budget. 
%control its sample actions in order to produce \Note{overall high confidence?} \circled{4} counts with highest confidence (i.e. lowest and bounded errors) under the energy budget 


%for each window, the sample quality (via the object counter choice) 
%and sample quantity (via the numbers of frames to process). 
%Across all windows of a horizon, these decisions collectively determine 
%the overall confidence in the emitted counts and the energy consumed in the \planwindow{}. 

The above theme sets \sys{} apart from various video analytics systems~\cite{noscope,focus,diva,videostorm,chameleon,vstore}. 
While prior systems optimize per-frame results (e.g., object labels), \sys{} is geared toward producing statistical results (i.e., aggregated counts) with bounded errors. 
While prior systems focused on cost/quality tradeoffs inherent in vision operators, 
%\sys{} in a much larger scope: 
\sys{} exploits higher-level tradeoffs between frame quantities and per-frame count errors, 
and therefore makes online decisions in the face of uncertain future.
\note{The above seems too abstract to me. Can we directly say Elf is the first to explore the joint trade-offs from both NN choice and frame sampling?}
Specifically:

\begin{comment}
Such sample planning is unaddressed in existing video analytics systems~\cite{noscope,focus,diva,videostorm,chameleon,vstore}. 
Those systems
1) consider no energy constraint, often assuming videos uploaded to centralized cloud to process;
2) provide only untrustworthy analytics results without bounded error, making the final results hard to interpret;
3) explores the tradeoffs only from inaccurate NNs, missing the opportunity from frame sampling.
\end{comment}

%Specifically, we address twofold challenges. 

%\paragraph{Deciding sample quality vs. quantity per window}
\noindent
%\textit{(1) Trade-off between sample quality and quantity per window} \hspace{1mm}
%\textbfit{(1) Characterizing sampling tradeoffs (space? parameter space?) per window} \hspace{1mm}
%\textbfit{(1) Per window: characterizing sampling tradeoffs (space? parameter space?)} \hspace{1mm}
%\textbfit{(1) Per window: characterizing energy/confidence (sampling action and outcome?)} \hspace{1mm}
\textbfit{(1) Per window: characterizing count actions and outcome} \hspace{1mm}
Of an aggregation window $w$, \sys{} faces a large space of \textit{count actions}:
%\st{i.e. the combinations of all counter choices and frame quantities,}
it not only chooses the number of frames to sample, 
but also chooses a counter, implemented as a neural network (NN), to process the frames. 
This is shown in Figure~\ref{fig:workflow}(b).
%Energy-expensive counters yield more \textit{exact} per-frame counts, and vice versa.
%(with lower errors in per-frame counts) 
%(yielding more exact per-frame counts) 
%(i.e. high quality per sample with low sample quantity) 
%or cheap counters 
%(with higher per-frame errors) 
%(yielding inexact per-frame counts). 
Different actions lead to disparate confidences in the aggregated count for window $w$ as well as disparate energy expenditures on $w$.
%(i.e. lower quality per sample with higher quantity). 
There is no silver-bullet action.
Notably, a more energy-expensive counter does not necessarily lead to higher confidence in the aggregated count:
%while it yields more exact per-frame counts, 
%while it incurs much lower errors in per-frame counts, 
%while the counter reduces errors in per-frame counts, \sys{} can afford processing much fewer frames for the whole window $w$.
while the counter may produce more exact per-frame counts, \sys{} can afford processing much fewer frames, hence the lower confidence. 

%much fewer frames can be afforded to sample by \sys{}. 
%\sys{} afford sampling fewer frames due to higher per-frame costs. 

%Among all the sample actions available for $W$, 
%we identify a \textit{energy/CI front} as the only sample actions that \sys{} should consider. 
Among all possible count actions for $w$, which ones should \sys{} consider? 
To answer this question, we identify an \textit{energy/CI front} as all the count actions that lead to the narrowest CIs at different energy expenditure levels.
% \textit{optimal} sample actions at different energy expenditures.
%as all the sample actions leading to the most confident count for the window (i.e., smallest CIs) given different energy allocations to that window.
%A window's energy/CI front contains all the \textit{optimal} sample actions.
%The front essentially reflects how a window's aggregated count gains additional confidence in response to energy investment. 
%The energy/CI front essentially reflects how the confidence to $W$'s aggregated count in return for energy investment, 
%providing the basis for \sys{} to plan sample actions. 
%\sys{} plan sample actions based on the energy/CI fronts of all windows.
%To \sys{}, the front reflects the \textit{return} of confidence on energy \textit{investment} for $W$. 
%Energy/CI fronts serve as the basis for \sys{} to plan sample actions. 
%Quantifying the energy/CI front requires to derive one unified CI by integrating two sources of errors: 
To quantify the energy/CI front, \sys{} integrates as one unified CI two errors: 
i) \sys{} sampling frames rather than processing all possible frames; 
ii) per-frame counts being inexact. 
% -- the one introduced by frame sampling and the one by inexact object counts on individual frames -- 
Prior AQP systems addressed the former~\cite{blinkdb,summarystore,olamr} but not the two integrated. 
\sys{} unifies the two errors with novel modeling and approximation, as will be discussed in \S\ref{sec:design-CI}.
%by i) modeling the latter error as a random variable independent of true object counts and time 
%and ii) a lightweight approximation of CIs which could have unwieldy forms~(\S\ref{sec:design-CI}). 

%We experimentally validate the resultant CIs.
%During integration, \sys{} exploits two key characteristics of the variable: independence from the true counts and independence from time. 
%We empirically validate the confidence intervals across a variety of videos. 

%As we will demonstrate, a window's energy/CI front primarily depends on the \Note{true?} object count in that window and the variation in the count.  

\noindent
%\textit{(2) Planning sampling across windows} \hspace{1mm}
%\textbfit{(2) Across windows: making heterogeneous count decisions on-the-go} \hspace{1mm}
\textbfit{(2) Across windows: making joint count decisions on the go} \hspace{1mm}
Of a window $w$, 
its energy/CI front reflects the confidence \textit{return} from the energy that \sys{} \textit{invests} in $w$. 
As we will empirically show, 
windows often have disparate energy/CI fronts.
%\st{primarily affected by their true object counts and the variations in the counts.}  
As a result, investing the same amount of energy on different windows often yields disparate CIs in their respective object counts. 
%\textit{returns} to the overall query confidence of a \planwindow{}.
%Towards maximizing the  %in a series of aggregated counts, 
As \sys{}'s objective is to maximize the overall confidence for a \planwindow{}, 
it must decide heterogeneous count actions for windows jointly, 
e.g., to invest more energy on windows where CI sees more substantial reduction. % significantly. 
%e.g., to invest more energy on windows where CI reduces more substantially. % significantly. 
%that will see higher CI reduction. 
 
%For instance, it may process more frames from windows exhibiting higher object counts and higher count variation, for which the additional energy expenditure results in higher improvement to the overall confidence. 

%For instance, it may invest extra energy on windows with higher object counts and higher count variation for denser sampling, and vice versa. 
%compared to windows with low object count / low variation, 
%the windows where the object count exhibits higher variation (standard deviation), result confidence sees higher improvement with energy investment (higher sampling quantity or quality). 
%the confidence quickly plateaus and sees diminishing return.  
%As different windows see varying benefits in response to energy allocation, 

To do so, 
\sys{} faces a dilemma between 
%the need for a \planwindow{}-wide view and decision timeliness: 
%the need for \planwindow{}-wide knowledge and the need for timely decisions: 
the needs for \textit{global knowledge} and for \textit{timely decisions}: 
i) to decide the optimal count action for a window $w$, 
\sys{} must compare the energy/CI fronts of all windows in the \planwindow{}; 
%\sys{} must compare its prospect of confidence gain (as reflected by $W$'s energy/CI front) to all other windows in the \planwindow{}; 
ii) to timely process $w$, 
\sys{} must decide the count action for $w$ prior to the window without seeing the \textit{future} windows.
To address this dilemma, 
%\sys{} makes on-the-go sampling decisions based on 
\sys{} \textit{predicts} the action count for each upcoming window 
based on the observation of past windows. 
Based on reinforcement learning, \sys{} mimics what an oracle planner, which (impractically) knows a \planwindow{}'s 
all past and future windows, \textit{would} decide. % with similar/same past windows.  
%We demonstrate that the learning predictor is as effective as predicting based on video heuristics,
%while relying on few assumptions on videos and no hand tuning of parameters. 



\sys{} runs on off-the-shelf embedded hardware.
%Raspberry Pi 4 (for image processing and NN inference) and OpenMV M7 (a low-power unit for image capturing).
Our tests on over 1000-hour real-world videos demonstrate \sys{}'s efficacy: 
with the energy level of a small solar panel, 
\sys{} continuously produces aggregated object counts that are only within 11\% of the truth counts.
At 95\% confidence level, their CI widths are as narrow as 17\% on average.
%\st{and XX\%  more compact compared to the baseline running only the most accurate NN counter.}
%On a typical battery of 150 Watt-hour, 
%\sys{} can operate for 15 days, producing aggregated counts with 21\% CI width on average.
%To reach typical CI width as target, \sys{} can reduce the overall energy by 4$\times$ on average and up to 12.5$\times$
%compared to the baseline running only the most accurate object detector.

We make the following contributions. 

\begin{myitemize}
\item 
%\textbf{new scenario}
%We make a case for pushing the geographic frontier of video analytics to  off-grid, autonomous cameras. 

\textit{The design space:}
We explore object counting on autonomous, energy-constrained cameras. 
We identify the central design problem as characterizing rich count actions and choosing them at run time. 

\item 
\textit{The problem formulation:}
%\textbf{problem formulation}
%We characterize sample actions and their outcomes as energy and confidence.
From the large space of count actions, 
we formulate an energy/CI front as the only actions that the camera should consider. 
%from which the camera should draw its sample actions. 
To quantify the front,
we propose novel techniques for unifying errors from multiple sources into a single CI.

\item 
%\textbf{novel mechanism}
%We design a learning-based planner for making heterogeneous sampling decisions. 
\textit{The runtime mechanisms:}
To plan count actions at run time, 
we design a novel, learning-based planner, which mimics the decisions made by an oracle under the same observation of past videos. 

%\begin{comment}
\item 
%\textbf{full prototype}
\textit{The implementation:}
We report a prototype \sys{}. 
Running on commodity hardware and with energy from a small solar panel, 
\sys{} continuously produces video summaries with high confidence. % with low, bounded errors. 
%\end{comment}

%To our knowledge, this the first time harnesses inaccurate NNs in answering object counting queries with \textit{bounded} errors. 

%\sys{} outperforms competitive alternatives by up to 10$\times$ energy saving.

\end{myitemize}

To our knowledge, \sys{} is the first system answering video object counting queries under energy constraint with bounded errors. 
At a higher level, it makes a case for pushing the geographic frontier of video analytics. 


==> intro-old.tex <==
% !TeX root = main.tex

\section{Introduction}\label{sec:intro}

IoT cameras are capable of producing colossal videos (16 GBs per camera per day) at low cost (\$20 each), 
therefore enabling a variety of video analytics~\cite{yogameena2017computer,karpagavalli2013estimating,
beymer1997real,lipton2015video,zhu2017online,
norouzzadeh2018automatically,mongeon2017busyness}.
%such as for public safety~\cite{yogameena2017computer,karpagavalli2013estimating,thangam2015crowd},
%traffic monitoring~\cite{beymer1997real,naphade2017nvidia,
%liu2016highway,hsieh2017drone},
%smart retailing~\cite{lipton2015video,mongeon2017busyness,
%zhu2017online,store-plan},
%and wild life monitoring~\cite{norouzzadeh2018automatically,parham2017animal,
%van2014nature,hodgson2016precision}. 
Yet, two major issues prevent AI-powered IoT cameras from being truly pervasive:
i) the need for wires, notably for continuous power supply, which 
raises barriers to camera deployment; 
ii) privacy concerns, as video footage is uploaded to the cloud and users often have limited, if any, ways for determining and controlling video content ~\cite{video-privacy-0,video-privacy-1,video-privacy-2,video-privacy-3,video-privacy-4,rtface,dufaux2010framework}.
\Note{as long as video leaves cameras, even to trusted edge, has privacy problem - side channel, etc}

%\textit{Infrastructure dependency}: 
%the need for power supply over wires and always-on network connectivity, raising the barrier of camera deployment. 
%\textit{Privacy concerns}: 
%unable to determine or control the content captured by IoT cameras, 
%users are increasingly concerned if video footage is uploaded to the cloud. \Note{cite}

\Note{should we identify and put scenarios here?} -- can we find some evidence showing many areas/regions are off the grid?

For these reasons, 
we have observed that IoT cameras are increasingly \textit{autonomous} with two notable trends. 
\begin{myitemize}
\item \textit{Energy independence.}
Cameras are capable of operating for long without external power supply. 
Major smart device vendors, e.g., Netgear, Reolink, Blink, have released popular battery-powered, ``wire-free'' cameras expected to work for months or years without battery replacement~\cite{reolink-argus,arlo-pro2,blink-indoor}.
Commercial cameras solely operating on solar energy also emerge~\cite{solar-camera,solar-AI}.
\Note{stress energy harvesting}

\item \textit{Compute independence.}
Cameras execute analytics, such as object detection, on device.
They only send concise summaries, e.g. object counts, to the cloud as requested by users. 
~\cite{solar-AI,JeVois,Vision-Kit,Firefly-DL}. 
Immediately after analytics they delete analyzed videos. 
\end{myitemize}

%The camera deployment and operation, under certain use cases, is evolving to be \textbf{autonomous}.
%On autonomous cameras, the video analytics runs purely on local device without any help from cloud/edge resources.
%The network resource is never used for video streaming, but only answering queries.
%Cameras operate on batteries without connecting to cable, which can be powered by solar energy or regularly re-charged.
%Energy is the main constrain of how video analytics can be carried out on autonomous cameras.
%Autonomous camera is privacy-friendly, because i) data never leaves camera, ii) data remains on camera for only a short period of time before permanently removed.

While easing deployment and assuring privacy, 
autonomous cameras are left with frugal resources, in particular  limited energy.
For example, a common solar panel (11.5"$\times$6"; harvesting 10Wh per day) can only supply
3\% of the energy needed by an embedded platform for object detection at 1 FPS~\cite{jetson-tx2}. 
One may wonder: can autonomous cameras perform any useful video analytics? 

\input{fig-workflow}

%To answer this question, we design \sys{}, a runtime system for \sysmodel{} to 
In this paper, we demonstrate that a resource-frugal autonomous camera can (periodically? continuously? estimate counts of object instance ...) execute ... a key class of video queries ... continuously counting objects in its video feeds with useful accuracy. 
Counting is a crucial query type for understanding video scenes, e.g., human crowd density and vehicle traffic.
They enable rich applications, including 
traffic monitoring~\cite{beymer1997real,naphade2017nvidia,
liu2016highway,hsieh2017drone},
public safety~\cite{yogameena2017computer,karpagavalli2013estimating},
wildlife monitoring~\cite{norouzzadeh2018automatically,parham2017animal,
van2014nature,hodgson2016precision},
and smart retailing~\cite{lipton2015video,mongeon2017busyness,
zhu2017online,store-plan}.
As shown in Figure~\ref{fig:workflow},
a counting query specifies an object class of interest, e.g., cars, 
and the length for each aggregation window, e.g., 30 mins. 
It expects a stream of aggregated object counts, one for each aggregation window elapsed.
The counts are approximate and are accompanied by confidence intervals (CIs), a common notion in 
approximate query processing (AQP)~\cite{blinkdb,summarystore,garofalakis2001approximate,olamr,
yan2014error,chakrabarti2001approximate}. 
The counts are stored on camera by default and can be retrieved on demand.

%By processing long-term videos, users expect counting results (number of object occurrence) within a time range (one hour). 



%For example, by counting the number of vehicles on intersections or highways, we can monitor the traffic for better city planning~\cite{beymer1997real,naphade2017nvidia,
%liu2016highway,hsieh2017drone}.
%By counting the number of persons in shopping malls, we can achive better
%public safety~\cite{yogameena2017computer,karpagavalli2013estimating} or store plan~\cite{lipton2015video,mongeon2017busyness,
%zhu2017online,store-plan}.
%Counting the number of different kinds of wild animals can help ecologists study their behavior~\cite{norouzzadeh2018automatically,parham2017animal,
%van2014nature,hodgson2016precision}.
%We will discuss query model in detail in $\S$\ref{sec:overview:query}. 



%\paragraph{How does \sys{} operate?}
\paragraph{The \sys{} design}
To execute counting queries on autonomous cameras, 
%the top goal is to best use limited energy for answering queries with highly confident results, i.e., bounded and low errors. 
%the top goal is:
% to best use limited energy for producing counts with high overall confidence, 
% e.g, with a minimum average error over a series of aggregated counts. 
% , i.e., with \textit{bounded} and \textit{low} errors. 
% to best use limited energy for producing highly confident counts, i.e., with \textit{bounded} and \textit{low} errors. \Note{clearly define goal}
we design a runtime system for \sysmodel{} called \sys{}. 
\sys{} operates under energy budget that is set by the OS (\st{or the user}) and replenished periodically (e.g. to reflect newly harvested energy). 
Note that the amount of energy per period could vary. 
The energy period is commonly implemented in energy-constrained \Note{harvesting} systems~\cite{goiri2012greenhadoop} 
giving them the essential headroom for planning energy use over long timespans. 

To count objects, \sys{} follows periodic sampling as in prior AQP systems \Note{cite}. 

As shown in Figure~\ref{fig:workflow}. 
%\sys{} processes sparse samples of image frames, as shown in Figure~\ref{fig:workflow}. 
over the course of each \aggwindow, \sys{} periodically wakes up and captures frames.
%At predefined (\Note{who defines?}) intervals 
it counts objects on captured frames by running neural nets (called NN object counters) on individual frames; 
\Note{refer back to figure 1}
based on per frame object counts, \sys{} derives per window \textit{aggregated} counts for all these windows.
\Note{still have to talk about frame capture \& processing}
\Note{merge the following}
During each \aggwindow, \sys{} periodically wakes up, captures, and stores video frames on local storage.
At the end of \aggwindow, \sys{} runs NN counters on the captured frames in \textit{batch} mode and generate aggregated counts.
All frames will be deleted once processed.
\Note{combine the following}
After materialization, \sys{} deletes all images for the $N$ windows. 
it also assures data privacy, as \sys{} never stores images older than a planning horizon.


\paragraph{The central problem: sample planning}
As its operation goal, 
\sys{} seeks to best use limited energy for producing counts with low, bounded errors. 
\Note{problem formulation}
\sys{} maximizes the mean confidence over all the aggregates. 
During operation, \sys{} decides for each window: 
the sample quality (via the choice of a NN counter) 
and sample quantity (via the numbers of frames to capture and to process). 
Across all windows of a horizon, these decisions collectively decide the horizon's query confidence (as the mean CI width) and its energy consumption. 

%The central goal of \sys{} is to best use limited energy for answering queries with high confidence and meaningful error estimation. 

%\paragraph{Deciding sample quality vs. quantity per window}
\noindent
%\textit{(1) Trade-off between sample quality and quantity per window} \hspace{1mm}
%\textbfit{(1) Characterizing sampling tradeoffs (space? parameter space?) per window} \hspace{1mm}
%\textbfit{(1) Per window: characterizing sampling tradeoffs (space? parameter space?)} \hspace{1mm}
\textbfit{(1) Per window: characterizing energy/confidence (sampling action and outcome?)} \hspace{1mm}

%The variety of NN-based object detectors open rich tradeoffs. 
%With the same amount of energy, 
Of a window, all possible sampling decisions constitute a large space. 
For instance, given the same amount of energy, 
\sys{} may run expensive counters on fewer frames (i.e. high quality with low quantity)
%(i.e. high quality per sample with low sample quantity) 
or cheap counters on more frames (i.e. low quality with high quantity); 
these decisions often yield disparate confidence (CI widths) for the window. 
%(i.e. lower quality per sample with higher quantity). 
There is no silver-bullet decision: 
with different amounts of energy is allocated to a window, 
the decision that lead to the highest confidence also varies. 

How should \sys{} navigate into such a space? 
We formulate 
a window's \textit{energy/CI front} as all the \textit{optimal} sample decisions that lead to the highest confidence answer (i.e. with lowest CIs) at a wide range of possible energy allocations.
%as the energy allocated to a window increases.
We demonstrate that a window's energy/CI front primarily depends on the object count and the count variation within the window, among other factors.  

A window's energy/CI front essentially reflects how a window's answer gain additional confidence in response to energy investment. 
As windows have different energy/CI fronts, they see disparate CI gain given the same energy investment. 
For instance, windows with higher object counts and higher count variation deserve denser sampling hence extra energy, and vice versa. 
compared to windows with low object count / low variation, 
the windows where the object count exhibits higher variation (standard deviation), result confidence sees higher improvement with energy investment (higher sampling quantity or quality). 
the confidence quickly plateaus and sees diminishing return.  

%Often, inaccurate NN counters triumph as they permits a large sample quantity at the cost of minor sample quality loss. 

The use of inaccurate NN counters further challenges \sys{} for presenting meaningful error for an aggregated count, as the error comes from two sources: 
i) that \sys{} samples frames rather than processing all available frames; 
and ii) that the object count on each sampled frames, as returned by inaccurate counters, 
is inexact. 
Prior AQP systems focus on the former but never cope with the two sources combined to our knowledge~\cite{blinkdb,summarystore,olamr}. 

To this end, \sys{} integrates errors from different sources
 (\S\ref{sec:design-CI})
 \sys{} quantifies two errors -- 
the one introduced by frame sampling and the one by inexact object counts on individual frames -- as one unified confidence metric. 
Our key idea is to model the latter error as a random variable. 
To integrate the errors, \sys{} exploits two key characteristics of the variable: independence from the true counts and independence from time. 
While the integrated error often has an unwieldy form, 
\sys{} uses lightweight approximation to produce  confidence intervals. 
We empirically validate the confidence intervals across a variety of videos. 


\noindent
%\textit{(2) Planning sampling across windows} \hspace{1mm}
\textbfit{(2) Across windows: making sample decisions on-the-go} \hspace{1mm}
As different windows see varying benefits in response to energy allocation, 
to maximize the \textit{overall} confidence %in a series of aggregated counts, 
\sys{} must pick heterogeneous sample qualities and quantities for individual windows. 

One may ... \sys{} shall make sample decisions \textit{in retrospect} at the end of a \planwindow{}, 
when it has knowledge of all the elapsed windows 
(estimated mean object counts and variations, energy/CI front);
and decide per-window sample quality/quantity by allocating energy to boost the overall confidence. 
However, doing so have two difficulties: 
i) the system would significantly delay materialization of aggregated counts, postponing it to the end of the current \planwindow{} (e.g. days); 
ii) as the system must determine the number of frames to capture per window at the beginning of that window which is much earlier than the offline decisions, 
excessive frame capture will burn out energy while 
insufficient sampling leaves surplus energy which result in low confidence in the emitted object counts. 
(misses the opportunity for higher confidence.)

Can \sys{} makes per-window sample decision at the beginning of each window, 
without seeing \textit{future} windows in the \planwindow{}, 
while still maximizing the overall confidence of the whole \planwindow{}?

%For instance, \sys{} may capture frames periodically during each aggregation window and only process frames at the end of each planning horizon, 

\Note{the following shall be rewritten. this should center on offline vs online tension. }

\paragraph{Executing queries: split-phase planning with probes} (\S\ref{sec:plan})
As shown in Figure~\ref{fig:workflow}, instead of deciding a horizon's sample qualities/quantities in one shot, 
\sys{} does so in two phases:
at the beginning of each window (\circled{1} the forward phase) and at the end of one entire planning horizon (\circled{2} the backward phase). 
Furthermore, as each window elapses, \sys{} processes a small fraction of frames, called \textit{probes}, as rough estimation of object count and variation in the window.

\Note{to be updated with RL}
In the forward phase for a window $W$, \sys{} decides sample  \textit{quality} for $W$; 
it does so by \note{reinforcement learning}.
\note{1-2 sentences explain how RL works here}
In the backward phase, \sys{} decides sample \textit{quantities} for all the windows enclosed in the planning horizon.  
\sys{} does so by allocating energy among the windows iteratively. 
With the finalized decisions, \sys{} reviews the forecast made in the forward phase and renews its knowledge. 

\sys{} materializes per window aggregated counts at the end of that window instead of the end of the \planwindow{}. 

%\sys{} decides sample quality and quantity for all windows in a planning horizon
%at the beginning of each window (a forward phase) and at the end of the entire planning horizon (backward phase), respectively. 
%In the forward phase for a window $W$, 
%\sys{} forecasts sample quantity to be decided in the backward phase for $W$ and 
%it then forecasts by learning from historic sampling decisions that were made under similar situations. 
%In the backward phase, \sys{} finalizes sample quantities for all {\aggwindow}s,  
%by allocating energy slices to them iteratively. 
%With the newly made sample decisions, \sys{} reviews the forward phase and renews its decision knowledge. 


\Note{how bad are we if we do naive online decisions per window?}


We build \sys{} atop off-the-shelf embedded hardware and test it on over 1000-hour real-world videos. 
%Raspberry Pi 4 (for image processing and NN inference) and OpenMV M7 (a low-power unit for image capturing).
Our results demonstrate its efficacy: 
powered by a typical solar panel (11.5"$\times$6"),
\sys{} can continuously produce aggregated object counts for every 30-min window.
The counts are only within 11\% of the ground truth counts; 
at 95\% confidence level, their CI widths are as narrow as 17\% on average.
On a typical battery of 150 Watt-hour, 
\sys{} can operate for 15 days, producing aggregated counts with 21\% CI width on average.
To reach typical CI width as target, \sys{} can reduce the overall energy by 4$\times$ on average and up to 12.5$\times$
compared to the baseline running only the most accurate object detector.


We make the following contributions. 

\begin{myitemize}
\item 
We identify the emerging scenario of running object counting query on autonomous cameras. 

\item 
\Note{formulate the problem}
We thoroughly investigate sampling decisions and their implications on energy consumption and query confidence. 
We propose a novel approach to integrate errors of multiple sources. 
To our knowledge, we are the first to harness inaccurate neural nets
in answering object counting queries with \textit{bounded} errors. 

\item 
We propose a novel mechanism, split-phase planning, for making heterogeneous sampling decisions for individual windows and resolving the tension of frame capturing/processing. 
\note{RL here}
%and allocates energy among them towards an overall optimal query confidence or energy consumption. 

\item
We build \sys{}, a runtime for executing counting with low errors under limited energy. 
Atop off-the-shelf embedded hardware, \sys{} demonstrates low errors and practical battery life to be useful. 

%\sys{} outperforms competitive alternatives by up to 10$\times$ energy saving.

\end{myitemize}



\Note{3 sentences set us apart from prior video analytics work. moved here. need more.}
The \textit{design goal} of \sys{} is to best use limited energy for answering queries with high confidence, i.e., with both bounded and low errors.
This problem is never addressed in existing video analytics systems~\cite{noscope,focus,diva,videostorm,chameleon,vstore} to our knowledge. 




% ----- Mengwei's ---- %
\begin{comment}
\note{Mengwei:}
\textbf{Key ideas}

\paragraph{1. A split-phase energy planning}
is deployed in \sys{} to fully utilize the rich trades-off from operator choice and cross-window disparity.
During online (forward) phase, \sys{} learns from historic knowledge to forecast the optimal decision likely to be made at offline, i.e., the most efficient NN for each \aggwindow, and how many frames needed to be processed.
The knowledge is maintained as a mapping from video characteristics (represented as mean and std of object counts over time, statistically sound) to the energy allocation to be received for such kind of {\aggwindow} from the total energy budget.
During offline (backward) phase, \sys{} judiciously allocates energy on different {\aggwindow}s to maximize the return in accuracy.
The allocation strategy is made at a global view to optimize the overall error from all {\aggwindow}s.
After the offline phase, the old knowlege will be renewed to adapt to changing goal and video characteristics.

\paragraph{2. To provide bounded error,} \sys{} is the first to treat the uncertainty from inaccurate NNs as a random variable, and statistically combine it with the error from sampling theory. 
We identify key characteristics of the error distribution introduced by inaccurate NNs, including its independence from ground truth and stability over time. 
\sys{} also approximates the combined, non-standard distribution in a computation-lightweight way without using simulation to obtain the bounded error.
\end{comment}

%\note{Mengwei:}
%\textbf{Key ideas}
%
%\paragraph{1. A split-phase energy planning}
%is deployed in \sys{} to fully utilize the rich trades-off from operator choice and cross-window disparity.
%During online (forward) phase, \sys{} learns from historic knowledge to forecast the optimal decision likely to be made at offline, i.e., the most efficient NN for each \aggwindow, and how many frames needed to be processed.
%The knowledge is maintained as a mapping from video characteristics (represented as mean and std of object counts over time, statistically sound) to the energy allocation to be received for such kind of {\aggwindow} from the total energy budget.
%During offline (backward) phase, \sys{} judiciously allocates energy on different {\aggwindow}s to maximize the return in accuracy.
%The allocation strategy is made at a global view to optimize the overall error from all {\aggwindow}s.
%After the offline phase, the old knowlege will be renewed to adapt to changing goal and video characteristics.
%
%\paragraph{2. To provide bounded error,} \sys{} is the first to treat the uncertainty from inaccurate NNs as a random variable, and statistically combine it with the error from sampling theory. 
%We identify key characteristics of the error distribution introduced by inaccurate NNs, including its independence from ground truth and stability over time. 
%\sys{} also approximates the combined, non-standard distribution in a computation-lightweight way without using simulation to obtain the bounded error.


==> noise.tex <==
\subsection{Taming operator error via image noise}
\note{This part will be removed}
As shown in Equation~\ref{eq:5} and~\ref{eq:6}, the CI width is directly related to the operator error, especially its standard deviation of mean value for each \aggwindow~($\sigma_{e}$). Larger operator error results in wider CI widths.

One of the main source of the operator error, of course, comes from the inaccuracy and uncertainty of NN itself.
However, we observe that the video temporal locality also exaggerates the error.
Assume the error of operator for each \textit{individual} frame follows a normal distribution $N(\mu_{d}, \sigma_{d})$.
If each frame is independent from each other, the distribution of mean value of {\aggwindow}s should follow another normal distribution with same mean ($\mu_d$) but much smaller standard deviation ($\sigma_d / \sqrt{n}$), where $n$ is the number of frames in each \aggwindow~\cite{mean-var}.

However, because of the temporal locality of video contents, the real variance of mean value is much larger than $\sigma_d / \sqrt{n}$. In other words, the frames within each \aggwindow{} are not representative of the frame distribution across all time.

To tame the variance caused by video temporal locality, \sys{} adds noise to the frames before processed by operator. It is based on two rationales:
(1) Noise can reduce the similarity among the image frames near in time.
(1) NNs have been proven to be robust to small noise.

As a small measurement study, we add Gaussian noise~\cite{gaussian-noise} to the images of Jackson videos.
\note{Show some results that it can help}.

==> opt.tex <==
\section{\sys{} Optimizations} \label{sec:opt}

\sys{} further applies two important optimization techniques.

\input{hw}

\input{noise}

==> recycle-abs.tex <==
%It is compelling to extend video analytics from urban areas to more diverse environments such as farms and underdeveloped regions. 
Rich applications will be enabled by extending video analytics beyond  urban areas to more diverse environments where cameras often stay off-grid and face constrained networks. 
To generate insights, cameras need to be \textit{autonomous}, executing analytics on device with limited energy. 

We present \sys{}, a runtime for autonomous cameras to produce video summaries as object counts. 
\sys{} centers on planning a camera's count actions under energy constraint, for which we contribute two novel techniques.
(1) \sys{} explores the rich action space spanned by the number of image frames to sample and the choice of per-frame object counters;
for the first time, it unifies the errors from both sources into one single bounded error. 
(2) To decide count actions at run time, 
\sys{} employs a learning-based planner that optimizes for past and future videos jointly while incurring no delay in materializing results. 
Tested with more than 1,000 hours of videos and realistic energy constraint, 
\sys{} continuously generates object counts that are only within 11\% of the true counts on average. 
Alongside the counts, \sys{} presents narrow error estimation shown to be bounded and up to 3.4$\times$ smaller than the baselines.
%It reduces the errors by up to 3.4$\times$ over baselines.
At a higher level, our experiences with \sys{} make a case for advancing the geographic frontier of video analytics. 
%At a higher level, \sys{} makes a case for pushing the geographic frontier of video analytics. 


==> recycle-design-CI.tex <==
% !TeX root = main.tex

\setlength{\belowdisplayskip}{5pt} \setlength{\belowdisplayshortskip}{1pt}
\setlength{\abovedisplayskip}{5pt} \setlength{\abovedisplayshortskip}{1pt}

\section{Integrating Multi-Source Errors}\label{sec:design-CI}

%\Note{much white space below can be compressed}
%\note{Check what distribution fits the video objects better.}

\paragraph{Approach Overview}
Recall from $\S$\ref{sec:overview}, \sys{} runs an NN counter on certain number of frames for each \aggwindow.
Based on the output of the counter (i.e., per-frame counts), \sys{} needs to derive the aggregated count (sum) and an associated CI.
Such derivation also is used to construct the energy/CI fronts as needed by our planner ($\S$\ref{sec:plan}).
The main challenge is to integrate the errors from two different sources: per-frame counting and sampling.
To this end, the key ideas of \sys{} are:
\begin{myitemize}
\itemsep0em 	
\item  Modeling the error from inaccurate per-frame counting as a random variable, and merge it with the traditional sampling theory.
\item  Approximating the combined, non-standard distribution in a computation-lightweight way without using simulation to obtain the CI.
\end{myitemize}

Note that \sys{} doesn't mix NN counters in one \aggwindow{}, as their outputs are difficult to be combined.
Our error-integration technique is validated in long-term real-world videos ($\S$\ref{sec:eval-perf}).

In the rest of section, we present the detailed formalization/deduction of our error-integration technique.

\noindent  \textbf{\textit{Input}}: the output counts of a given NN counter on a set of frames ($X_i, i \in [1,2,...n]$). The frames are uniformly sampled within the target \aggwindow.

\noindent  \textbf{\textit{Output}}: an estimation of the ground-truth mean object counts ($\mu$) within the \aggwindow, including the mean and a CI with confidence level $\alpha$.

According to the statistics theory~\cite{intro-stats}, we have
\begin{equation}\label{eq:1}
\frac{\bar{X}-\mu_x}{S/\sqrt{n}} \thicksim T_{n-1}
\end{equation}
where $\bar{X}$ and $S$ are the mean and standard deviation of $X$, $\mu_x$ is the mean of NN counter output on all the frames in \aggwindow, and $T_{n-1}$ is the Student's t-distribution with \textit{n - 1} degrees of freedom.
\revise{Noting that the above theory is valid regardless of the distribution of $\mu_x$ according to central limit theorem.}

However, the NN counter introduces extra error from the ground-truth mean ($\mu$).
%The reason is that on a frame,  operator's object count does not always agree with ground truth.
%Thus, We need to model the error to map our observations to the ground truth.
%One way is to use prediction interval (PI)~\cite{pred-interval} to estimate the error introduced by operator on each sample. However, existing approaches to generate PIs such as model ensemble~\cite{pi-ensemble} incurs too much computation overhead.
To deal with this challenge, our approach is to \textit{treat the error of inaccurate NN counter as a random variable that follows a certain distribution, and integrate it with the distribution of sampling result.}
Intuitively, the error is proportional to the ground-truth mean value: more objects appear during the \aggwindow, more FP and FN tend to be made by the NN counter. 
Thus, we model the error as the ratio between $\mu$ and $\mu_x$ ($\mu / \mu_x \thicksim E_1$).
However, we observe that, when the absolute value of $\mu$ is too small, the error (ratio) is often very large (outliers).
Including those outliers in the overall error distribution will result in very high distribution variance.
To eliminate the impacts from those outliers, we set a threshold $\theta$: when $\mu$ is smaller than the threshold, we model the error as linear offset between the mean of ground truth and NN counter ($\mu - \mu_x \thicksim E_2$). In practice, we can use $\bar{x}$ to estimate whether $\mu$ is larger than the threshold $\theta$.

% \begin{equation}\label{eq:2}
% E =
%   \begin{cases}
%     \mu \div \mu_x \thicksim N(\mu_{e1}, \sigma_{e1}^2)      & \quad \text{if } \mu > \theta\\
%     \mu - \mu_x \thicksim N(\mu_{e2}, \sigma_{e2}^2)  & \quad \text{if } \mu \leq \theta
%   \end{cases}
% \end{equation}

We have two key observations about the error distribution of NN counters:
\begin{myitemize}
\item Error distribution is stable over time.
We measure the error of two NN counters (\code{YOLOv2} and \code{ssd mobilenet-v2}) on the video stream Jackson.
The stream has two separated 1-week video clips with 1-month interval (captured at the first week of May. 2019 and Jun. 2019).
The results show that the Bhattacharyya coefficient~\cite{bhattacharyya1943measure}
% \footnote{A common metric to measure the similarity between distributions.}
between the errors of two weeks are 0.93 and 0.86 for two NN counters, respectively.
As a result, we can profile the error distribution for once (e.g., when camera is installed) and use it later on.
% Notice that, unlike some prior work~\cite{noscope,diva} that trains the specialized NNs based on the test video, NN counters are trained on generic dataset (COCO) without specialization.
\item Error is independent from $X$, as confirmed by chi-square test~\cite{intro-stats} based on the videos we collected. It helps us to simplify the integration of two distributions.
\end{myitemize}


Thus, we have the new distributions ($V1$ and $V2$) of target $\mu$ as following:
\begin{equation}\label{eq:3}
\mu =
   \begin{cases}
     (\bar{x} + S/\sqrt{n} \cdot t) \times e_1 \thicksim V1 & \quad \text{if } \bar{x} > \theta\\
     (\bar{x} + S/\sqrt{n} \cdot t) + e_2  \thicksim V2 & \quad \text{if } \bar{x} \leq \theta
   \end{cases}\\
\end{equation}
\[
   here: t \thicksim T_{n-1}, e_1 \thicksim E_1, e_2 \thicksim E_2
\]
 
The distribution of NN counter error ($E$) can be regarded as a punishment to the resultant CI. Larger error indicates larger $\sigma(E)$, and so more uncertain $V$ distribution, finally results in wider CI. We use $\mu_{e1}, \mu_{e2}$ to denote the mean of $E_1, E_2$.
Based on the above, we have the CI of $\mu$ as following.
\begin{flalign*}
&    \text{if } \bar{x} > \theta: CI = [\bar{x} \times \mu_{e1} - v_{1,\alpha},\bar{x} \times \mu_{e1} + v_{1,\alpha}] \\
&    \text{if } \bar{x} \leq \theta: CI = [\bar{x} + \mu_{e2} - v_{2,\alpha},\bar{x} \times \mu_{e2} + v_{2,\alpha}]
\end{flalign*}
\begin{flalign*}
where \quad & {P(|V_1-\bar{X}\times\mu_{e1}|\leq v_{1, \alpha})=\alpha \%}\\
& {P(|V_2-\bar{X} - \mu_{e2}|\leq v_{2, \alpha})=\alpha \%}
\end{flalign*}
The CI width, i.e., $v_{1, \alpha}$ and $v_{2, \alpha}$, can be derived through Monte Carlo simulation~\cite{monte-carlo}: randomly picking the same number ($N$) of samples from t-student distribution and NN counter's error distribution ($e_1,e_2$) respectively, then combine them as Equation~\ref{eq:3}. The results, denoted as $(y_1,y_2,...,y_N)$, should follow the target distribution of $\mu$. The CI width, taking $v_{1, \alpha}$ as an example, can be obtained as the smallest $w$ that makes the range $[\bar{x} \times \mu_{e1} - w, \bar{x} \times \mu_{e1} + w]$ cover at least $\alpha \% \times N$ data points out of $(y_1,y_2,...,y_N)$.

\paragraph{Approximating $\mu$ distribution} In practice, one disadvantage of using Monte Carlo simulation to obtain the CI is that it involves intensive computations, especially when it needs to be repeatedly computed in our sampling planning ($\S$~\ref{sec:plan}).
Fortunately, we observe that the distribution of $\mu$ is close to normal distributions with similar CDF (cumulative distribution function). Thus, we can approximate the CI width ($v_{1, \alpha}, v_{2, \alpha}$) by treating $V_1,V_2$ as normal distributions with mean $E(\mu)$ and standard deviation $\sigma(\mu)$.


Based on Equation~\ref{eq:3}
% and the observation that error distribution of NN counter is independent from $\mu_x$,
we can derive the mean and standard deviation of $\mu$ as following. Here, $\mu_{e1}, \mu_{e2}$ are the mean of the NN counter's error distribution $E_1, E_2$, and $\sigma_{e1}, \sigma_{e2}$ are their standard deviation.
\begin{gather}
\begin{aligned}
\bar{x} > \theta: \quad
\sigma^2(\mu) & = (\sigma^2(u_x) + \bar{X}^2)(\mu_{e1}^2+\sigma_{e1}^2) - \bar{X}^2\mu_{e1}^2 \\
\bar{x} \leq \theta: \quad
\sigma^2(\mu) & = \sigma^2(u_x) + \sigma_{e2}^2\\
where: \quad
\sigma^2(u_x) & = \frac{S^2}{n} \sigma(t_{n-1}) = \frac{S^2(n-1)^2}{n(n-3)^2}
\end{aligned}
\label{eqt:numerical_scheme1}
\raisetag{20pt}
\end{gather}
\begin{comment}
\begin{equation}\label{eq:4}
\begin{split}
\bar{x} > \theta: \quad
\sigma^2(\mu) & = (\sigma^2(u_x) + \bar{X}^2)(\mu_{e1}^2+\sigma_{e1}^2) - \bar{X}^2\mu_{e1}^2 \\
\bar{x} \leq \theta: \quad
\sigma^2(\mu) & = \sigma^2(u_x) + \sigma_{e2}^2\\
where: \quad
\sigma^2(u_x) & = \frac{S^2}{n} \sigma(t_{n-1}) = \frac{S^2(n-1)^2}{n(n-3)^2}
\end{split}
\end{equation}
\end{comment}
%\begin{equation}\label{eq:4}
%E(\mu) =
%   \begin{cases}
%     \bar{X} \times \mu_{e1} & \quad \text{if } \bar{x} > \theta\\
%     \bar{X} + \mu_{e2} & \quad \text{if } \bar{x} \leq \theta
%   \end{cases}\\
%\end{equation}
%\begin{equation}\label{eq:5}
%\sigma^2(\mu) =
%   \begin{cases}
%     (\sigma^2(u_x) + \bar{X}^2)(\mu_{e1}^2+\sigma_{e1}^2) - \bar{X}^2\mu_{e1}^2 & \quad \text{if } \bar{x} > \theta\\
%     \sigma^2(u_x) + \sigma_{e2}^2 & \quad \text{if } \bar{x} \leq \theta
%   \end{cases}\\
%\end{equation}
%\[
%here: \sigma^2(u_x) = \frac{S^2(n-1)^2}{n(n-3)^2}
%\]
As $V_1, V_2$ are approximated as normal distributions:
\begin{equation}\label{eq:5}
v_{1, \alpha}, v_{2, \alpha} = z_{\alpha/2} \sigma(\mu)
\end{equation}
%\begin{equation}\label{eq:5}
%\begin{split}
%& V_1, V_2 \thicksim N(E(\mu), \sigma^2(\mu)) \\
%& \Rightarrow \frac{v_1 - E(\mu)}{\sigma(\mu)}, \frac{v_2 - E(\mu)}{\sigma(\mu)} \thicksim N(0, 1) \\
%& \Rightarrow v_{1, \alpha}, v_{2, \alpha} = z_{\alpha/2} \sigma(\mu)
%\end{split}
%\end{equation}
The approximation also helps us to understand how different factors affect the CI widths $v_{1, \alpha}, v_{2, \alpha}$.
It also shows how the CI width reduces when the number of samples increases.
It is used to guide \sys{} to perform energy allocation across multiple windows ($\S$\ref{sec:plan}).


\paragraph{Convert mean to aggregation (sum)}
The above shows how to get the mean object count, e.g., ``average number of cars crossing the road \textit{each second}''.
To convert it to aggregation count, e.g., ``total number of cars crossing the road within half hour'', we only need to multiply the mean by window size, e.g.,
$[0.5 \pm 0.1] \rightarrow [900 \pm 180]$ with half-hour window size.



%\subsection{Extending to Advanced Queries}
%
%\note{Remove this part}
%
%The above explains how \sys{} estimates the distribution and the CI of the mean value for a specific time window. It's easy to extend the approach to more generic query types.
%
%\noindent $\bullet$ \textbf{Across multiple {\aggwindow}s}: when a query covers multiple {\aggwindow}s, simply putting all the samples from those windows together will result in inaccurate estimation. The reason is that the sampling strategy becomes biased (no longer random) as different {\aggwindow}s may have different number of samples according to our sampling strategy.
%Instead, \sys{} averages the distributions (derived in Equation~\ref{eq:3}) across every \aggwindow{}, then calculates the CI through the new distribution in the same way as single \aggwindow.
%We put the details of how to derive CI of multiple {\aggwindow}s in Appendix B.
%
%\noindent $\bullet$ \textbf{comparison queries}: \sys{} currently supports linear comparison, e.g., whether the mean number of cars during $T_i$ is $\alpha$ times larger than $T_j$? Based on Equation~\ref{eq:3}, \sys{} constructs the mean distribution $V_i$ and $V_j$ for those two {\aggwindow}s, respectively. The question can be answered as ``Yes'' with confidence $P(V_{i} - \alpha V_{j} > 0)$, or ``No'' with confidence $P(V_{i} - \alpha V_{j} \leq 0)$, depending on the actual confidence number.
%\note{Put an appendix}

==> tab-hw.tex <==
\begin{table}[]
\footnotesize
\begin{tabular}{l|L{4.2cm}|L{1cm}}
\hline
\textbf{Hardware} & \textbf{Specifications} & \textbf{job} \\ \hline
OpenMV M7~\cite{M7-camera} & ARM Cortex M7 at 216 MHz, 512KB RAM, OV7725 image sensor & capture \\ \hline
Raspberry Pi 4~\cite{rpi4} & ARM Cortex A72 at 1.5GHz, 2GB RAM & process \\ \hline
\end{tabular}
\caption{Hardware of \sys{}}\label{tab:hw}
\end{table}

==> tab-params.tex <==
% !TeX root = main.tex

\begin{table}[t!]
\centering
\includegraphics[width=0.49\textwidth{}]{figs/tab-params.pdf} 
%\missingfigure[figwidth=6cm]{Kernel support}
\caption{A summary of \sys{} parameters for query and system, respectively. \textbf{XXXX update the table XXXX}}
\label{tab:params}
\end{table}

==> todo2.tex <==

\vspace{5pt}
\textbf{Disclaimer}: 
The authors have consulted the PC chairs on the paper's suitability for MobiSys, and were encouraged to submit.

